Extensions of submanifold theory to non-real settings, with applications

In this thesis, we study extensions of the theory of Riemannian submanifolds in two directions. First, we will show how Riemannian geometry and submanifold theory in particular, can be generalized using the notion of 'Rinehart spaces', and it will be demonstrated how the developed framework unifies some existing and new flavours of Riemannian geometry over different ground rings. In the second part of the thesis, we give a description of holomorphic Riemannian submanifold theory where complex numbers fully replace the role of the real numbers as ground field, and show how this can be applied to reveal direct connections between the submanifolds of so-called Wick-related pseudo-Riemannian spaces.

==> chapters/abstract/abstract.tex <==
\chapter{Abstract}\label{ch:abstract}

In this thesis, we study extensions of the theory of Riemannian submanifolds in two directions. First, we will show how Riemannian geometry and submanifold theory in particular, can be generalized using the notion of `Rinehart spaces', and it will be demonstrated how the developed framework unifies some existing and new flavours of Riemannian geometry over different ground rings. In the second part of the thesis, we give a description of holomorphic Riemannian submanifold theory where complex numbers fully replace the role of the real numbers as ground field, and show how this can be applied to reveal direct connections between the submanifolds of so-called Wick-related pseudo-Riemannian spaces.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/abstractnl.tex <==
\chapter*{Beknopte samenvatting}

In deze thesis bestuderen we uitbreidingen van de theorie over Riemannse deelvari\"eteiten in twee richtingen. Allereerst laten we zien dat Riemannse meetkunde, en deelvari\"eteitentheorie in het bijzonder, veralgemeend kan worden gebruikmakend van het concept `Rinehartruimtes', en we zullen laten zien hoe dit bestaande en nieuwe soorten van Riemannse meetkunde over verschillende grondringen in \'e\'en theorie verenigt. In het tweede deel van de thesis beschrijven we holomorf Riemannse deelvari\"eteitentheorie, waarin complexe getallen volledig de rol van de re\"ele getallen als grondveld overnemen, en we laten zien hoe dit kan worden toegepast om directe verbanden bloot te leggen tussen deelvari\"eteiten van zogenoemde Wickgerelateerde pseudo-Riemannse ruimtes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/preface/preface.tex <==
\chapter*{Dankwoord}                                  \label{ch:preface}

Voor de totstandkoming van deze thesis zijn er een aantal personen die ik wil bedanken.

Allereerst wil ik Franki Dillen bedanken. Hij heeft mij immers de mogelijkheid geboden om aan de KU Leuven mijn doctoraat te maken. Spijtig genoeg is vanwege zijn ongelukkige overlijden diens begeleiding maar van korte duur geweest. Ik heb Franki eigenlijk vooral leren kennen uit alle mooie verhalen die ik na zijn overlijden over hem gehoord heb.

Ik dank Joeri Van der Veken voor de excellente wijze waarop hij de taak van Franki heeft overgenomen. Hij heeft mij altijd veel vrijheid en vertrouwen gegeven om nieuwe onderzoeksrichtingen te verkennen, maar ook adequaat bijgestuurd wanneer dat nodig was. Ik heb zijn begeleiding dan ook bijzonder gewaardeerd.

Verder wil ik uiteraard de leden van de jury hartelijk bedanken. Zij hebben mij in verschillende stadia van de thesis zeer geholpen met al hun waardevolle opmerkingen. Maar ook buiten de leden van de jury zijn er veel collega's die ik dankbaar ben voor de hulp die ze bij mijn onderzoek geboden hebben, alsook juist de nodige afleiding daarvan. In het bijzonder wil ik daarom nog bedanken: Henri Anciaux, Nastassja Cipriani, Bart Dioos, Alfonso Garmendia, Alexander Lemmens, Francisco Torralbo, Leopold Verstraelen en Ori Yudilevich.

Buiten mijn collega's wil ik nog bedanken: Jasmijn en Adeline voor de extra dimensie die ze aan mijn doctoraatsperiode hebben gegeven, Biyun om gedurende mijn doctoraat aan twee zulke leuke dochters geboorte te geven, mijn ouders, broer en zus voor hun voortdurende steun op de achtergrond, en tenslotte nog de verzorgsters van kinderdagverblijf De Kabouterberg, omdat ik niet weet hoe ik zonder hun toegewijde zorg voor Jasmijn en Adeline mijn thesis had kunnen voltooien.
%\instructionspreface


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}

